Gamma-ray emission from spectrally resolved cosmic rays in galaxies

Cosmic rays (CRs) are ubiquitous in the interstellar medium (ISM) of nearby galaxies, but many of their properties are not well-constrained. Gamma-ray observations provide a powerful tool in this respect, allowing us to constrain both the interaction of CR protons with the ISM and their transport properties. To help better understand the link between observational signatures and CR physics, we use a series of magneto-hydrodynamical (MHD) AREPO simulations of isolated galaxies performed using spectrally-resolved CR transport in every computational cell, with subsequent gamma-ray emission calculated using the CRAYON+ (Cosmic RAY emissiON) code. In each of our simulated halos, modelling the energy-dependent spatial diffusion of CRs leads to a more extended distribution of high-energy (~100 GeV) gamma rays compared to that predicted by a 'grey' steady-state model, which is especially visible in the corresponding emission maps and radial profiles. Despite this, the total gamma-ray spectra can often be well approximated by the steady-state model, although recovering the same spectral index typically requires a minor variation of the energy dependence of the diffusion coefficient. Our simulations reproduce the observed spectral indices and gamma-ray spectra of nearby star-forming galaxies and also match recent observations of the far infrared--gamma-ray relation. We find, however, that the spectrally resolved model yields marginally smaller luminosities for lower star formation rates compared to grey simulations of CRs. Our work highlights the importance of modelling spectrally resolved CR transport for an accurate prediction of spatially resolved high-energy gamma-ray emission, as will be probed by the upcoming Cherenkov Telescope Array observatory.

==> Makefile <==
# Makefile to produce the article.
PDFLATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: pdflatex
LATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: latex
DVIPS  =  dvips
FIGURES = 

.PRECIOUS: $(FIGURES)

default: main.pdf

%.pdf :  $(FIGURES) %.tex
	$(PDFLATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	make clean

%.ps :  $(FIGURES) %.tex
	$(LATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(LATEX) $*.tex
	$(LATEX) $*.tex
	$(LATEX) $*.tex
	$(DVIPS) -o $*.ps $*.dvi
	ps2pdf $*.ps
	make clean

figures/%.eps: figures/%_raw.eps figures/%.tex
	(cd figures; latex $*.tex; \
	dvips -E -o $*.eps $*.dvi; \
	perl -ane '{ s/%%BoundingBox: [-0-9]+/%%BoundingBox: 135/g; print}' $*.eps > tmp.eps; \
	mv tmp.eps $*.eps; \
	rm -f *.dvi *.log *.aux)

clean:
	rm -f *.log *.toc *.aux *.dvi *.bak *.blg *.obj *.out

realclean:
	rm -f *.log *.toc *.aux *.dvi *.obj *.bak *.bbl *.blg *.brf \
              *.pdf *.ps */*.ps *~ */*~ *.bak */*.bak 









